On Using Information Retrieval to Recommend Machine Learning Good Practices for Software Engineers

Machine learning (ML) is nowadays widely used for different purposes and in several disciplines. From self-driving cars to automated medical diagnosis, machine learning models extensively support users' daily activities, and software engineering tasks are no exception. Not embracing good ML practices may lead to pitfalls that hinder the performance of an ML system and potentially lead to unexpected results. Despite the existence of documentation and literature about ML best practices, many non-ML experts turn towards gray literature like blogs and Q&A systems when looking for help and guidance when implementing ML systems. To better aid users in distilling relevant knowledge from such sources, we propose a recommender system that recommends ML practices based on the user's context. As a first step in creating a recommender system for machine learning practices, we implemented Idaka. A tool that provides two different approaches for retrieving/generating ML best practices: i) an information retrieval (IR) engine and ii) a large language model. The IR-engine uses BM25 as the algorithm for retrieving the practices, and a large language model, in our case Alpaca. The platform has been designed to allow comparative studies of best practices retrieval tools. Idaka is publicly available at GitHub: https://bit.ly/idaka. Video: https://youtu.be/cEb-AhIPxnM.

==> secs/4_tool.tex <==

\section{Preliminary Empirical Study}

We conducted a preliminary study aimed at (i) identifying which IR model provides the best results in \approach and (ii) whether the  practices retrieved by \approach are useful to users.  In particular, we investigated the following research questions:

\begin{itemize}
	\item \textbf{RQ$_1$}: \emph{What is the IR-model used in \approach that provides the best precision and recall?}
	\item \textbf{RQ$_2$}: \emph{How useful are the results retrieved by \approach?}
\end{itemize}


To answer \textbf{RQ$_1$}, manually created a ground set composed of 85 queries and the corresponding practices relevant to the queries.  Afterward, one author used three versions of  our approach with different IR models: \approach$_{(LDA)}$, \approach$_{(VSM)}$, and \approach$_{(BM25)}$. Finally, by following the ground truth, and the retrieved results we computed Precision@k and Recall@k, both  from 1 to 10. To answer  \textbf{RQ$_2$}, we asked undergraduate students (relevance of the use of students shown in previous studies \cite{feldt2018four, falessi2018empirical})  of a computer science program to write a query on \approach and evaluate the usefulness of the retrieved results with a 5-stars scale. The students were recruited by using convenience sampling over the authors' social networks. Note that the student has basic knowledge of ML.

\subsection{What is the IR-model used in \approach that provides the best precision and recall?}
On a search engine, precision and recall are essential quality measures since the user is expecting not only that the results are related to the query but also that the answers they are looking for can be reached on the results that the engine provides. In our case, these two measures were calculated at k from 1 to 10. As a result, better performance on precision than recall was found for the three algorithms. \figref{figrq1_results} shows the Precision@k and Recall@k for the 85 queries. 
On average, the best algorithm was \textit{BM25}, followed by \textit{VSM}, and finally, \textit{LDA}. The latter had a significantly lower performance than the other two algorithms, which can be explained by the length of the documents, which need to be longer for an efficient prediction of the topics and, therefore, of the ranking.  \textit{BM25} is considered the most appropriate model for \approach, especially for its satisfactory precision performance throughout all k.

\begin{figure}
	\centering
	\includegraphics[width=0.8\columnwidth]{imgs/rq1_precision.pdf}
	\includegraphics[width=0.8\columnwidth]{imgs/rq1_recall.pdf}
	
	\caption{Precision@k and Recall@k of different IR models in \approach}
	\label{figrq1_results}
\end{figure}

\subsection{How useful are the results retrieved by \approach?}
Based on the results for \textbf{RQ$_1$}, as the selected IR model, with Sparck, by the study participants. Concerning the study procedure, first, each participant was told about the main objectives of \approach. Then, we gave them access to the web page and told them to navigate through it. We asked them to explore the three functionalities and emphasized that on the main view, they had to write a query related to an ML task and rate (using a 1-5 stars scale) the practices retrieved by \approach. The results are the following: 5$\star$ (8 participants), 4$\star$ (7 participants), 3$\star$ (8 participants), and 2$\star$ (3 participants), which account for an average rating of 3.77.  
Analyzing more thoroughly the cases with rate=2, we identified three possible causes. First, the queries rated with two are the longest. Second, there are discrepancies between words on the query and a documents: that come from typos or the ways the users expresses themselves. For example, among the queries rated with 2, it is found that the user wrote 'cross-validation,' and in the documents, this term appears as 'cross-validation'. The last factor was that our corpus needed to be larger to supply overspecified queries. For example, 'Use of cross-validation for logit model' would not find an answer in our collection.
